BiasMap: Leveraging Cross-Attentions to Discover and Mitigate Hidden Social Biases in Text-to-Image Generation

Bias discovery is critical for black-box generative models, especiall text-to-image (TTI) models. Existing works predominantly focus on output-level demographic distributions, which do not necessarily guarantee concept representations to be disentangled post-mitigation. We propose BiasMap, a model-agnostic framework for uncovering latent concept-level representational biases in stable diffusion models. BiasMap leverages cross-attention attribution maps to reveal structural entanglements between demographics (e.g., gender, race) and semantics (e.g., professions), going deeper into representational bias during the image generation. Using attribution maps of these concepts, we quantify the spatial demographics-semantics concept entanglement via Intersection over Union (IoU), offering a lens into bias that remains hidden in existing fairness discovery approaches. In addition, we further utilize BiasMap for bias mitigation through energy-guided diffusion sampling that directly modifies latent noise space and minimizes the expected SoftIoU during the denoising process. Our findings show that existing fairness interventions may reduce the output distributional gap but often fail to disentangle concept-level coupling, whereas our mitigation method can mitigate concept entanglement in image generation while complementing distributional bias mitigation.

==> mitigation_algo.tex <==
2. for denoise loop
3. irrelevant, mention in passing
4. CFG expansion talk about first [explain epsilon!], + significance of 2 + editing prompts
5. irrelevant, again single line
6. we pass to unet (with gradient monitoring already mentioned)
7. ovam capture mentioned in prelim, can shorten
8. softtopk mention paper + reason + exactly what is done
9. we motivate our loss with iou, instead of (what was done before) + intuitively why should this make sense? + why does iou need to be continuous and differentiable for our work + any improvements in matrix ops or TC? [can bring comparisons to how fuzzy assignment is better than hard assignment]
10. standard pipeline step? not relevant
11. epsilon not defined anywhere! mention how updated. a surface level discussion on guidance
12-15: together
16: we finally inject bias gradient as 
rest are standard shit.
